Practical Experience Report: The Performance of Paxos in the Cloud

This experience report presents the results of an extensive performance evaluation conducted using four open-source implementations of Paxos deployed in Amazon's EC2. Paxos is a fundamental algorithm for building fault-tolerant services, at the core of state-machine replication. Implementations of Paxos are currently used in many prototypes and production systems in both academia and industry. Although all protocols surveyed in the paper implement Paxos, they are optimized in a number of different ways, resulting in very different behavior, as we show in the paper. We have considered a variety of configurations and failure-free and faulty executions. In addition to reporting our findings, we propose and assess additional optimizations to existing implementations.

==> ospaxos.v1.tex <==
%!TEX root =  main.tex
\section{Open-source Paxos libraries}
\label{libs}
In this section, we describe three open-source Paxos implementations with emphasis on their properties relevant to our performance evaluation. 
In the discussion, we distinguish between ``slow" and ``fast" acceptors. 
%
%Paxos is known to remain operational despite the failure of $f$ acceptors. 
%Therefore, progress is ensured 
%
%
%An acceptor is slow acceptor is an acceptor that is not respondent within an expected interval. 
%In modern datacenters, a process is often collocated with other processes where resources such as networking and processing powers are shared among them. In addition, machines in a datacenter may have different specifications. 
%These are two of a variety of reasons that can cause performance differences among the acceptors where some appear to be slower.
A slow acceptor is an acceptor that is not respondent within an expected interval. 
In modern datacenters, a process is often collocated with other processes where resources such as networking and processing powers are shared among them. In addition, machines in a datacenter may have different specifications. 
These are two of a variety of reasons that can cause performance differences among the acceptors where some appear to be slower.


Paxos requires a majority quorum for progress, that is, it remains operational despite the failure of $f$ acceptors. 
%
%is known to remain operational despite the failure of $f$ acceptors. 
However, we argue that failures can still affect the performance of Paxos if acceptors are subject to non-uniform resource allocation. OpenReplica, S-Paxos, and Libpaxos are reasonably similar in the way they implement Paxos. 
Nevertheless, due to the differences in their communication styles, they differ in (a) how flow control is handled in the presence of non-equivalent acceptors and (b) how their performance is affected by failures. We describe next these differences.

%extensions and optimizations
\subsection{OpenReplica}
OpenReplica is an open-source library implemented in Python\footnote{https://pypi.python.org/pypi/concoord} that enables automatic replication of user-provided objects~\cite{Altinbuken12}. 
At its core lies a Paxos implementation that makes the library fault-tolerant. OpenReplica is composed of a set of replicas and a set of acceptors. Replicas are the processes that replicate an object. One of the replicas also plays the role of the leader in Paxos. To submit their requests, clients connect to the pool of replicas and OpenReplica ensures that the requests are forwarded to the leader to be ordered. Replicas deliver and execute the sequence of requests, in an order dictated by instance identifiers. Replicas also respond to the clients. 

The leader in OpenReplica uses non-blocking I/O to communicate with the acceptors. If the transmission of a message to an acceptor fails, the leader retries the transmission until it succeeds. If an acceptor is slow in processing the packets that it has received from the leader, its incoming buffer gradually fills up. This is an example of a situation where non-blocking communication with such an acceptor may fail at the leader. The leader who fails to transmit a message to the slow acceptor will retry sending the message until it succeeds. During this interval, the leader devotes a fraction of its processing power to resubmissions and we can expect a reduction in the proposing speed and thus in the overall performance. Moreover, the slow acceptor who is not contributing to new instances can clear its incoming buffer so that the leader can eventually resume their communication. If during this interval one of the fastest acceptors leaves the acceptor set, we can expect a further reduction in performance if a majority-quorum of acceptors is not available immediately. 
%The reduction should be worse at the beginning of this interval since the  

\subsection{S-Paxos}
S-Paxos~\cite{spaxos} is implemented in Java\footnote{https://github.com/nfsantos/S-Paxos}
and is composed of a set of replicas who also play the role of the acceptors. One of the acceptors assumes the role of the leader. The key idea in S-Paxos is to distribute the tasks of request reception and dissemination among all the replicas. 
A client selects a replica arbitrarily and submits its requests to it. 
After receiving a request, a replica forwards it (or possibly a batch of requests) to all the other replicas. 
A replica that receives a forwarded request sends an acknowledgement to all the other replicas. 
When a replica receives $f+1$ acknowledgements, it declares the request stable. 
As in classic Paxos, the leader is responsible for ordering requests; differently from Paxos, ordering is performed on request ids. 
An acceptor considers an instance closed after receiving $f+1$ Phase~2B messages. 
All the replicas execute all the requests but only the replica who receives the request responds to the client. 
S-Paxos makes a balanced use of CPU and network resources. 
Many messages must be exchanged before a request can be ordered. 
Due to the high number of messages exchanged, S-Paxos is CPU-intensive and demonstrates its best performance when deployed on multi-core machines.  

\textbf{.. reasoning is not convincing}\\
S-Paxos uses blocking I/O for the communications among replicas. As mentioned earlier, a replica forwards batches of requests to all the other replicas. If a replica is not fast enough in removing packets from its incoming buffers the communications with it will block. Faster acceptors can not transfer more batches to the slow replica and therefore we expect the performance of the system to follow the speed of the slowest replica. Thus if a fast acceptor decelerates amid the execution we don't expect any reduction in the performance. However, since S-Paxos is designed around the idea of having more acceptors to have higher throughput, as the acceptor set shrinks, performance may experience some decrease. 
%Therefore, we can expect that performance will not be substantially affected by the crash of a fast acceptor. 

\subsection{Libpaxos}

Libpaxos is implemented in C.\footnote{https://bitbucket.org/sciascid/libpaxos}
It distinguishes the roles of acceptors, learners, and proposers. 
Proposers execute Phase~1 and Phase~2 of Paxos and do not assume the role of an acceptor. To submit their requests, clients connect directly to the proposers. Acceptors communicate with the proposer(s) and also with the learners. Acceptors send their Phase~2B messages, including the agreed value, to the proposer(s) and also to the learners. 
Upon receiving $f+1$ Phase~2B messages from the acceptors the learners and the proposer(s) declare an instance as decided. The learners deliver instances following instance identifiers. 
The proposer(s) do(es) not communicate directly with the learners. 

Processes in Libpaxos communicate through non-blocking buffered I/O provided by the libevent library.\footnote{http://libevent.org} Since besides sending Phase~2B, an acceptor also sends values to the learners and proposer(s) the amount of data transferred through its outgoing links is higher than the amount of data received through its incoming links.\footnote{Notice that the only processes from which an acceptor \emph{receives} data is the proposers.} It is possible for the data in the outgoing buffers of a slow acceptor to be accumulated without being actually transmitted. As a consequence, this acceptor eventually lags behind and the instances get decided with the participation of the faster acceptors in which the outgoing buffers do not pile up. 

Thus we expect the performance in Libpaxos to be determined by the performance of the faster acceptors. Were the outgoing buffers of the acceptors used equal to or less than its incoming buffers, similar to OpenReplica we would expect the performance to be driven by the speed of the communication of the leader to the slow acceptor. If amid the execution a fast acceptor decelerates or crashes, performance may suffer a sudden reduction as a majority-quorum may not be available immediately and the slow acceptor needs to clear the expired data from its outgoing buffers before contributing to an instance. As the slow acceptor continues to empty its buffers new instances can not be decided. During this period the proposer, who is not receiving $f+1$ Phase~2B messages, is expected to also reduce its proposing rate.

%...Before the period, 
%...During the period, 
%...After this period, we expect Libpaxos to operate at the speed of the slower acceptor.

%In all the experiments that we have performed with Libpaxos  there is one proposer, one learner, a set of clients, and a set of acceptors whose size is specified separately for each experiment. 
% and is available for download at~\cite{lugano-paxos}.\footnote{All the communications are one-to-one and TCP-based in all the libraries.}
%\section{Flow control}
%The inclusion of a relatively slower acceptor in the acceptor set of Paxos reveals different behaviors in the aforementioned libraries. In the followings we discuss each one separately. \\
%\noindent \textbf{OpenReplica.} The leader in OpenReplica uses non-blocking IO to communicate with the acceptors. However, if sending a Phase~2A message to an acceptor fails the leader enters a loop and  resends the message until it succeeds. If an acceptor is slower in removing packets from its buffers, sending additional Phase~2A messages to it will cause the leader to enter the aforementioned loop frequently. During these intervals as the leader spends a fraction of its time busy-trying inside this loop, its proposing speed reduces and the slower acceptor makes time to empty its buffers. Meanwhile only faster acceptors participate in closing the instances. OpenReplica arbitrates between intervals in which the throughput increases (when all the acceptors have similar speed) and decreases (when the slow acceptor can not keep up with the rest). Therefore if at the middle of the execution a faster acceptor leaves, performance will not be affected dramatically. \\

%\noindent \textbf{S-Paxos.} S-Paxos uses blocking IO for the communications among replicas. As mentioned earlier a replica forwards batches of requests to all the other replicas. Since a slower acceptor is not fast enough in removing packets from its socket buffers, eventually its buffers will fill up and the communications with it will block. As the faster acceptors can not transfer more batches to the slower replica, the system operates at the speed of the slower replica. Therefore, if at the middle of this situation a fast acceptor leaves, performance will not be affected dramatically. From the beginning, S-Paxos adapts its performance to the capacity of the slow acceptor.\\

%\noindent \textbf{U-Ring Paxos}---\\

%\noindent \textbf{Libpaxos.} Libpaxos uses non-blocking IO through a buffered write option for the communications among the processes. In Libpaxos it is the acceptors that communicate with the learners to transfer the values and Phase~2B messages. When an acceptor is slower, its sending buffers grow faster compared to the other acceptors. However, since the other acceptors are faster, instances are decided without the participation of the slower acceptor. Thus Libpaxos operates at the speed of the faster acceptors. On the negative side, if at the middle of the execution a fast acceptor leaves the performance drops to zero as the slower acceptor has never had the time to empty its buffers. It takes a while until the buffers are emptied, during which new instances can not be decided. After this period Libpaxos operates at the speed of the slower acceptor. \\
% and is available for download at~\cite{spaxos-lib}.

%\subsection{U-Ring Paxos}
%
%In U-Ring Paxos all the processes are distributed on a logical ring. It is composed of a set of acceptors among which one plays the role of the leader. Clients select an arbitrary acceptor and submit their requests to it. If received by a non-leader acceptor, a request is forwarded along the ring until it reaches the leader who proposes it to Paxos. Any process along the ring records the request. Are the learners/ replicas, the same processes as acceptors?.... 
%
%U-Ring Paxos is developed in Java and is available for download at~\cite{uringpaxos}.




==> table.tex <==
\begin{table*}[ht]
\caption{This table contains the specifications for the configurations we have evaluated the three libraries in. The leader in OpenReplica represents the replica,  A1 in S-Paxos is represented by the leader. and the concept of learner only exists in Libpaxos.}
\label{table:configs}
%{
\centering
\small
%{\tiny
%\resizebox{\textwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|} \hline
Configuration &  Type & Environment &  Leader & A1 & A2 &A3 & Learner\\  \hline \hline
(a) & Homogeneous & LAN & Small  &Small & \begin{tabular}[x]{@{}c@{}}\\Small\\\\\end{tabular} & \begin{tabular}[x]{@{}c@{}}\\Small\\\\\end{tabular} & Small \\ \hline

(b) & Heterogeneous & LAN  & Small & Small & \begin{tabular}[x]{@{}c@{}}\\Small\\\\\end{tabular} & \begin{tabular}[x]{@{}c@{}}\\Micro\\\\\end{tabular} & Small\\ \hline

(c) & Heterogeneous & LAN &Large & Small & \begin{tabular}[x]{@{}c@{}}\\Small\\\\\end{tabular} & \begin{tabular}[x]{@{}c@{}}\\Micro\\\\\end{tabular}	& Small \\ \hline

(d) & Homogeneous & WAN &Small & Small & \begin{tabular}[x]{@{}c@{}}\\Small\\\\\end{tabular} & \begin{tabular}[x]{@{}c@{}}\\Small\\\\\end{tabular} & Small\\ \hline
\end{tabular}
%}
%}
\end{table*}

